Many-Objective Evolutionary Influence Maximization: Balancing Spread, Budget, Fairness, and Time

The Influence Maximization (IM) problem seeks to discover the set of nodes in a graph that can spread the information propagation at most. This problem is known to be NP-hard, and it is usually studied by maximizing the influence (spread) and, optionally, optimizing a second objective, such as minimizing the seed set size or maximizing the influence fairness. However, in many practical scenarios multiple aspects of the IM problem must be optimized at the same time. In this work, we propose a first case study where several IM-specific objective functions, namely budget, fairness, communities, and time, are optimized on top of the maximization of influence and minimization of the seed set size. To this aim, we introduce MOEIM (Many-Objective Evolutionary Algorithm for Influence Maximization) a Multi-Objective Evolutionary Algorithm (MOEA) based on NSGA-II incorporating graph-aware operators and a smart initialization. We compare MOEIM in two experimental settings, including a total of nine graph datasets, two heuristic methods, a related MOEA, and a state-of-the-art Deep Learning approach. The experiments show that MOEIM overall outperforms the competitors in most of the tested many-objective settings. To conclude, we also investigate the correlation between the objectives, leading to novel insights into the topic. The codebase is available at https://github.com/eliacunegatti/MOEIM.

==> bak/old_text.tex <==
% \begin{itemize}
% \item Gnutella 6301 20,777 Directed - Epinions 75,879 508,837 Directed \cite{pham2019competitive} (LT MODEL and $\tau=5)$
% \item Cora 2708 5278 - email-Eu-Core 1005 4170 - Facebook ego/combined 4039 8832 \cite{gong2023influence} In this paper, we adopted the IC model which is widely used. To test different cases, we have the seed set size k=4, the propagation probability $p \in {0.05, 0.1, 0.15}$, and the time limit $\tau=5$. Under other parameter settings, such as $k \in {4, 8, 12}$, $p \in {0.05, 0.1, 0.15}$ and $\tau \in {2, 5, 8}$ our method can achieve the best results.
% \item DBLP We then extracted the largest connected component of this graph, resulting in 53, 307 nodes and 288, 864 edges \cite{stoica2020seeding} - IC, $p=0.01$ and $p=0.1$
% \end{itemize}
